Enabling Design Methodologies and Future Trends for Edge AI: Specialization and Co-design

Artificial intelligence (AI) technologies have dramatically advanced in recent years, resulting in revolutionary changes in people's lives. Empowered by edge computing, AI workloads are migrating from centralized cloud architectures to distributed edge systems, introducing a new paradigm called edge AI. While edge AI has the promise of bringing significant increases in autonomy and intelligence into everyday lives through common edge devices, it also raises new challenges, especially for the development of its algorithms and the deployment of its services, which call for novel design methodologies catered to these unique challenges. In this paper, we provide a comprehensive survey of the latest enabling design methodologies that span the entire edge AI development stack. We suggest that the key methodologies for effective edge AI development are single-layer specialization and cross-layer co-design. We discuss representative methodologies in each category in detail, including on-device training methods, specialized software design, dedicated hardware design, benchmarking and design automation, software/hardware co-design, software/compiler co-design, and compiler/hardware co-design. Moreover, we attempt to reveal hidden cross-layer design opportunities that can further boost the solution quality of future edge AI and provide insights into future directions and emerging areas that require increased research focus.

==> raw_comments.tex <==
Editor
Comments to the Author:
Please note that two of the reviewers have pointed towards some fundamental limitation of this article. Please address their comments and resubmit for the second round of reviews.


Reviewer: 1

Recommendation: Reject

Comments:
The paper presents a summary of design methodologies, technologies, benefits, challenges and trends associated with the emerging domain of Edge AI.

Major Comments
1.      There are already plenty of surveys and papers emphasizing the current trends and the current state-of-the-art in Edge AI. How is this paper different? For example, with respect to references [4]-[6] presented in the paper. Most of the technical content described in this article are already present in other surveys. The reviewer could not find any new value in this article.
2.      As a survey paper, there should be at least some figures, numbers, or studies illustrating the research problems in the field of Edge AI. For example, the computing capabilities, power budgets of edge nodes vs. server platforms could be easily depicted with graphs to provide a more comprehensive and clearer understanding of the domain, with a solid motivation.
3.      There could be more figures to explain various sections of the paper, such as a use-case diagram depicting the architecture of nodes deployed in an application.
4.      Instead of merely discussing the edge devices in the text, graphs with potential results could help the reader better understand the complexities and performance of such systems. The same goes for all other aspects, such as software development, HW/SW co-design, benchmarking, etc.

Minor Comments
1.      Shouldn’t the title say, “future trends for Edge AI”, in plural, considering that the application domain is highly heterogeneous, which can lead to an emergence of multiple trends.
2.      The keywords and the complete list of authors are missing in the submission page.
3.      There are quite a few grammatical mistakes in the paper. Please proofread.
4.      The chain of argumentation is confusing at times, for example, the second paragraph of section 1.
5.      The section numbers could be included in fig.1.
6.      Instead of using “the work” for explaining references [4]-[6], either use “<LastNameofFirstAuthor> et al. [4] provide …” or “The work presented in [5] …”.


Additional Questions:
1. How relevant is this manuscript to the readers of this periodical? Please explain your rating in the Detailed Comments section.: Relevant

1. Please summarize what you view as the key point(s) of the manuscript and the importance of the content to the readers of this periodical. If you don't have any comments, please type No Comments.: The paper presents a summary of design methodologies, technologies, benefits, challenges and trends associated with the emerging domain of Edge AI.

2. Is the manuscript technically sound? Please explain your answer in the Detailed Comments section.: No

3. What do you see as this manuscript's contribution to the literature in this field? If you don't have any comments, please type No Comments.: The paper presents a summary of design methodologies, technologies, benefits, challenges and trends associated with the emerging domain of Edge AI.

4. What do you see as the strongest aspect of this manuscript? If you don't have any comments, please type No Comments.: No Comments

5. What do you see as the weakest aspect of this manuscript? If you don't have any comments, please type No Comments.: It is a survey, but the reviewer could  not find any new value of this article, as there is a plenty of surveys on this topic already. Also, quantitative information is missing from this article, see detailed comments below.

1. Are the title, abstract, and keywords appropriate? Please elaborate in the Detailed Comments section.: Yes

2.  Does the manuscript contain title, abstract, and/or keywords?: Yes

3. Does the manuscript contain sufficient and appropriate references? Please elaborate in the Detailed Comments section.: References are sufficient and appropriate

4. Does the introduction state the objectives of the manuscript in terms that encourage the reader to read on? Please explain your answer in the Detailed Comments section.: No

5. How would you rate the organization of the manuscript? Please elaborate in the Detailed Comments section.: Could be improved

6. Is the manuscript focused? Please elaborate in the Detailed Comments section.: Could be improved

7. Is the length of the manuscript appropriate for the topic? Please elaborate in the Detailed Comments section.: Could be improved

8. Please rate the readability of this manuscript in the Detailed Comments section.: Readable - but requires some effort to understand

Please rate the manuscript. Explain your choice in the Detailed Comments section.: Poor


Reviewer: 2

Recommendation: Accept If Certain Minor Revisions Are Made

Comments:
Summary: This paper provides a survey on Edge AI’s challenges, methodologies, and future trends. It is very timely and informative, and I think it would be useful to anyone interested in the general topic of edge AI. The authors do a good job in motivating the problems and discussing the current methodologies addressing them. I do not have any major comments but have some suggestions that could improve the survey.

Comments:

-       I do think the survey could use more high-level visualizations. For example, Section 4.1 could show some high-level ideas for model compression and design. This could make it easier for the reader to understand the high level goals.

-       Figure 2 needs more information to understand what the figure is trying to demonstrate. What are the axes? Descriptions for (a) and (b) should be in the caption, etc.

-       “Distributed edge training has been largely…” -> “Distributed edge training has largely…”


Additional Questions:
1. How relevant is this manuscript to the readers of this periodical? Please explain your rating in the Detailed Comments section.: Very Relevant

1. Please summarize what you view as the key point(s) of the manuscript and the importance of the content to the readers of this periodical. If you don't have any comments, please type No Comments.: This paper provides a survey on Edge AI’s challenges, methodologies, and future trends.

2. Is the manuscript technically sound? Please explain your answer in the Detailed Comments section.: Yes

3. What do you see as this manuscript's contribution to the literature in this field? If you don't have any comments, please type No Comments.: This paper provides a survey on Edge AI’s challenges, methodologies, and future trends.

4. What do you see as the strongest aspect of this manuscript? If you don't have any comments, please type No Comments.: It is very timely and informative, and I think it would be useful to anyone interested in the general topic of edge AI. The authors do a good job in motivating the problems and discussing the current methodologies addressing them.

5. What do you see as the weakest aspect of this manuscript? If you don't have any comments, please type No Comments.: No Comments

1. Are the title, abstract, and keywords appropriate? Please elaborate in the Detailed Comments section.: Yes

2.  Does the manuscript contain title, abstract, and/or keywords?: Yes

3. Does the manuscript contain sufficient and appropriate references? Please elaborate in the Detailed Comments section.: References are sufficient and appropriate

4. Does the introduction state the objectives of the manuscript in terms that encourage the reader to read on? Please explain your answer in the Detailed Comments section.: Yes

5. How would you rate the organization of the manuscript? Please elaborate in the Detailed Comments section.: Satisfactory

6. Is the manuscript focused? Please elaborate in the Detailed Comments section.: Satisfactory

7. Is the length of the manuscript appropriate for the topic? Please elaborate in the Detailed Comments section.: Satisfactory

8. Please rate the readability of this manuscript in the Detailed Comments section.: Easy to read

Please rate the manuscript. Explain your choice in the Detailed Comments section.: Excellent


Reviewer: 3

Recommendation: Author Should Prepare A Major Revision For A Second Review

Comments:
Summary:

This is a survey paper on the topic of EdgeAI from different perspectives including software, hardware, hardware and software co-design, and design automation methodologies for creating effective solutions. The paper

Pros:

+ Edge AI is an important topic
+ Paper covers reasonable ground and made some good choices about the overall organization.

Cons:

- Technical exposition can be improved.
- Some important related work and problem perspective is missing.
- Could use more figures to better illustrate solution approaches.
- Could provide more quantitative results comparing different solution approaches in the trade-off space

Detailed comments:

1. I would have liked to see a good problem setup covering all the relevant details.

What type of AI problems are being solved?
- Type of input data: image, video, text, time-series, graph
- Type of output: simple output from a small set of classes (classification) or structured output (images, 3D shapes, sequences, and graphs)
- Type of neural networks: CNNs for images; Sequence-to-sequence models; and Graph neural networks

Much of the current work in Edge AI problem space falls in the category of images as input, classification problem, and CNNs as AI model.

What are the different classes of EdgeAI applications and how do their requirements in terms of different design metrics change? Which applications need further investigation?

2. Security is an important design metric for Edge AI solutions. This paper completely ignores this aspect of the problem and relavant work.

3. There is good amount of prior work on the design of specialized DNNs for edge platforms: MobileNets, SqueezeNets, ShuffleNets, ChannelNets, SlimNets etc. I couldn't locate this discussion.

https://arxiv.org/abs/1704.04861
https://arxiv.org/abs/1602.07360
https://papers.nips.cc/paper/7766-channelnets-compact-and-efficient-convolutional-neural-networks-via-channel-wise-convolutions.pdf
https://arxiv.org/abs/1707.01083
https://arxiv.org/abs/1808.00496

4. In the software and hardware/software co-design, an important solution approach is that of adaptive inference (using simpler networks for simple inputs and complex networks for harder inputs dynamically).

Conditional Deep Learning for energy-efficient and enhanced pattern recognition. DATE 2016: 475-480
Trading-Off Accuracy and Energy of Deep Inference on Embedded Systems: A Co-Design Approach. IEEE Trans. Comput. Aided Des. Integr. Circuits Syst. 37(11): 2881-2893 (2018)
Designing adaptive neural networks for energy-constrained image classification. ICCAD 2018
PareCO: Pareto-aware Channel Optimization for Slimmable Neural Networks. CoRR abs/2007.11752 (2020)
Design and Optimization of Energy-Accuracy Tradeoff Networks for Mobile Platforms via Pretrained Deep Models. ACM Trans. Embed. Comput. Syst. 19(1): 4:1-4:24 (2020)
AdaScale: Towards Real-time Video Object Detection using Adaptive Scaling. MLSys 2019

5. It would be nice to provide high-level illustrative figures to capture different classes of solution approaches. This will greatly help the reader and improve the impact of the paper.

6. One critical drawback of this paper is that it doesn't discuss any quantitative aspects of different solution frameworks and approaches within to help the reader understand the trade-off space in terms of different design metrics. Subsequently, a good discussion about how some of these solutions can be synergistically combined to further improve the achievable Pareto front will greatly help the reader and also the EDA community in pursuing solutions to further push the Pareto front.


==> sections/figure-all-works.tex <==


\begin{table*}[]
    \centering
    \begin{tabular}{c | c | l }
    
    \hline
    \textbf{Domain} & \multicolumn{2}{c}{\textbf{Description}} \\
    \hline
    
     \textcolor{blue}{Low-precision} & 
     \multicolumn{2}{l}{ \textcolor{blue}{E2-train: Training state-of-the-art cnns with over 80\% energy savings \cite{wang2019e2}}} \\
     \textcolor{blue}{Edge Training} & 
     \multicolumn{2}{l}{\textcolor{blue}{ShiftAddNet: A Hardware-Inspired Deep Network \cite{you2020shiftaddnet}}} \\
     & \multicolumn{2}{l}{ \textcolor{blue}{FracTrain: Fractionally Squeezing Bit Savings Both Temporally and Spatially for Efficient DNN Training~\cite{fu2020fractrain}}} \\
     & \multicolumn{2}{l}{\textcolor{blue}{HALO: Hardware-aware learning to optimize~\cite{li2020halo}}} \\
     & \multicolumn{2}{l}{\textcolor{blue}{Ultra-Low Precision 4-bit Training of Deep Neural Networks~\cite{sun2020ultra}}} \\
     & \multicolumn{2}{l}{\textcolor{blue}{A new MRAM-based process in-memory accelerator for efficient neural network training with floating point precision~\cite{wang2020new}}} \\
     & \multicolumn{2}{l}{\textcolor{blue}{Hybrid 8-bit floating point (HFP8) training and inference for deep neural networks~\cite{sun2019hybrid}}} \\
     & \multicolumn{2}{l}{\textcolor{blue}{TinyTL: Reduce Memory, Not Parameters for Efficient On-Device Learning~\cite{cai2020tinytl}}} \\
     
     \hline
     
    Software     & Model  &  VecQ: a DNN quantization method minimizing vector loss as the quantization objective function \cite{gong2020vecq}. \\    
    Development  & Compression & Channel gating (CG): dynamically determine whether computing full or partial channels \cite{hua2019channel}. \\
                 &              &  Precision gating (PG): dynamically determines which features to run in half or full precision \cite{zhang2020pg}. \\    
                 &              &  Outlier channel splitting: duplicates outlier channels and halves the values to improve DNN accuracy \cite{zhao2019ocs}. \\    
                  &              & CMix-NN: an open-source mixed low bit-width inference library for quantized networks on MCUs \cite{capotondi2020cmix}. \\ 
                  & & \textcolor{blue}{SlimNets: model compression through weight pruning, low rank factorization, and knowledge distillation \cite{oguntola2018slimnets}} \\
                                  
    \cline{2-3}
                & Model       & \textcolor{blue}{Compact model designs: MobileNet~\cite{howard2017mobilenets, sandler2018mobilenetv2}, ShuffleNet~\cite{zhang2018shufflenet} , SqueezeNets~\cite{iandola2016squeezenet}, ChannelNets~\cite{gao2018channelnets}, } \\
                
                 & Design        & SkyNet: a hardware-aware bi-directional DNN design approach to deliver hardware-efficient DNNs \cite{zhangskynet}. \\    
                 
                 &               & MNasNet: a reinforcement learning based NAS that incorporates DNN latency into the search space \cite{tan2019mnasnet}. \\    

                 &              & Proxyless-NAS: a differentiable latency-aware NAS with reduced memory usage during training \cite{cai2018proxylessnas}. \\    
                 &              & EEG-TCNet: a low complexity temporal convolutional network (TCN) for embedded classification \cite{ingolfsson2020eeg} \\    
                 &              & HadaNet: a DNN based on unitary group convolutions (UGConvs) using Hadamard transform \cite{zhao2019ugconv}. \\    
    \cline{2-3}
                 & \textcolor{blue}{Adaptive}     &  
                 \textcolor{blue}{Conditional deep learning for energy-efficient and enhanced pattern recognition \cite{panda2016conditional}} \\

                 & \textcolor{blue}{Inference}     &  
                \textcolor{blue}{ Trading-off accuracy and energy of deep inference on embedded systems: A co-design approach \cite{jayakodi2018trading}}\\    
                
                & & \textcolor{blue}{ Designing adaptive neural networks for energy-constrained image classification \cite{stamoulis2018designing}} \\
                
                & & \textcolor{blue}{ PareCO: Pareto-aware Channel Optimization for Slimmable Neural Networks \cite{chin2020pareco} } \\
                
                & & \textcolor{blue}{ Design and Optimization of Energy-Accuracy Tradeoff Networks for Mobile Platforms~\cite{jayakodi2020design} } \\
                
                & & \textcolor{blue}{Adascale: Towards real-time video object detection using adaptive scaling \cite{chin2019adascale} } \\
                 
     \hline
     
    Hardware     & CPU/GPU & Tensaurus: an accelerator that is capable of accelerating mixed sparse-dense matrix operations \cite{srivastava2020tensaurus}. \\    
    Development  &               & Dynamic power selection: a Dynamic Voltage and Frequency Scaling (DVFS) based power management \cite{di2020idleness}. \\    
                 &               & Q-EEGNet: an accelerator for EEGNet \cite{lawhern2018eegnet} on an ultra-low power RISC-V based System-on-Chip \cite{schneider2020q}. \\
                 &               & XpulpNN: a set of extensions to the RISC-V ISA for energy efficiency of low-bitwidth quantized DNNs \cite{garofalo2020xpulpnn}. \\    
                 &               & Fann-on-mcu: an open-source toolkit for energy-efficient DNN inference at ARM and RISC-V platforms \cite{wang2020fann}. \\ 
                 &               & PULP-NN: an open-source optimized library for low-bit DNN inference on RISC-V platforms \cite{garofalo2020pulp}. \\
    \cline{2-3}
                 & FPGA   & TCN accelerator: an architecture template supporting temporal convolution networks inference on FPGA \cite{carreras2020optimizing}. \\
                 &              & BNN accelerator: the first binarized neural network accelerator on FPGA synthesized from C++  \cite{zhao2017accelerating}. \\    
                 &              & T-DLA: the first instruction-based open-source accelerator for ternarized DNNs on embedded FPGAs \cite{chen2019t}. \\   
                 &              &
                 Low bit-width acceleration: a design flow of accelerating hybrid low bit-width DNNs on FPGAs~\cite{wang2018design}. \\
                 
                 &              & HybridDNN: a framework for building Spatial/Winograd hybrid DNN accelerators on FPGA \cite{ye2020hybrid}. \\    
                 &              & Sparse DNN accelerator: a configurable sparse DNN inference accelerator on FPGA \cite{huang2019accelerating}. \\    
    \cline{2-3}             
                 & ASIC   & CG \cite{hua2019channel} accelerator: an RTL-level accelerator using channel gating to exploit DNN dynamic sparsity \cite{hua2019boosting}. \\ 
                 &              & ChewBaccaNN: a binary CNN accelerator chip using various memory- and power-efficient technologies \cite{andri2020chewbaccann}. \\   
                 &      & DianNao Family: a series of ML acceleration chips ranging from data center to edge scale \cite{chen2016diannao}. \\
                 &      & Eyeriss: an energy-efficient deep convolutional neural network (CNN) accelerator chip \cite{chen2016eyeriss}. \\
 
     \hline
     
     Software- &   \multicolumn{2}{l}{FPGA/DNN co-design: the first fully simultaneous and automatic FPGA/DNN co-design framework \cite{hao2018deep, hao2019fpga}} \\   
     hardware &       \multicolumn{2}{l}{FNAS: a reinforcement learning based FPGA-aware NAS with FPGA design space exploration during search \cite{jiang2019accuracy}} \\    
     Co-design &        \multicolumn{2}{l}{NAIS: the first work to discuss simultaneous neural architecture and implementation co-search for various hardware \cite{hao2019nais}. } \\    
     &        \multicolumn{2}{l}{EDD: a differentiable NAIS formulation and framework targeting arbitrary hardware platforms \cite{li2020edd}} \\    
      &        \multicolumn{2}{l}{ NASAIC: the first work on multi-task neural architecture and heterogeneous ASIC accelerator design co-exploration \cite{yang2020co}.} \\    
          
    &        \multicolumn{2}{l}{ \textcolor{blue}{Patdnn: Achieving real-time DNN execution on mobile devices with pattern-based weight pruning \cite{niu2020patdnn} }} \\    
    &        \multicolumn{2}{l}{ \textcolor{blue}{ PCONV: The Missing but Desirable Sparsity in DNN Weight Pruning for Real-Time Execution on Mobile Devices \cite{ma2020pconv}} } \\
    &       \multicolumn{2}{l}{ \textcolor{blue}{ CocoPIE: Making Mobile AI Sweet As PIE--Compression-Compilation Co-Design Goes a Long Way \cite{liu2020cocopie} } } \\
    &       \multicolumn{2}{l}{ \textcolor{blue}{ {RTMobile: Beyond Real-Time Mobile Acceleration of RNNs for Speech Recognition} \cite{dong2020rtmobile} } } \\
    
    &        \multicolumn{2}{l}{ \textcolor{blue}{MCUNet: Tiny Deep Learning on IoT Devices~\cite{ji2020mcunet}}} \\
    &       \multicolumn{2}{l}{\textcolor{blue}{Lite Transformer with Long-Short Range Attention~\cite{Wu2020LiteTransformer}}} \\
    &       \multicolumn{2}{l}{\textcolor{blue}{HAT: Hardware-Aware Transformers for Efficient Natural Language Processing~\cite{hanruiwang2020hat}}} \\
    &       \multicolumn{2}{l}{\textcolor{blue}{Searching Efficient 3D Architectures with Sparse Point-Voxel Convolution~\cite{tang2020searching}}} \\
    &       \multicolumn{2}{l}{\textcolor{blue}{Once for All: Train One Network and Specialize it for Efficient Deployment~\cite{cai2020once}}} \\
    &       \multicolumn{2}{l}{\textcolor{blue}{TSM: Temporal Shift Module for Efficient Video Understanding~\cite{lin2019tsm}}} \\
          
     \hline
     
     Scalable           &        \multicolumn{2}{l}{MLModelScope: a scalable benchmark platform for deep learning workloads on various hardware with profiling traces \cite{dakkak2018mlmodelscope, li2020design}.} \\
     
     Benchmarking       &        \multicolumn{2}{l}{XSP: an automated tool to analyze integrated workload performance metrics of models, frameworks, and GPUs \cite{li2019acrossstack}.} \\
     
     \hline
     
     Design     &   \multicolumn{2}{l}{DNNBuilder: an automatic tool with DSE for building high-performance DNN hardware accelerators on FPGAs \cite{zhang2018dnnbuilder}.}   \\
     
     Automation & 
     \multicolumn{2}{l}{AutoDNNChip: an automated DNN chip performance predictor and design builder for both FPGAs and ASICs \cite{xu2020autodnnchip}.} \\
     
     &   \multicolumn{2}{l}{SystemC modeling: an automated SystemC generation and DSE flow through polyhedral model-based techniques \cite{zuo2015polyhedral}. }  \\
    
    &   \multicolumn{2}{l}{RIP: an ILP-based framework to accelerate tasks by partitioning hardware/software under power and area constraints \cite{zuo2017accurate}. }  \\
    
    &    \multicolumn{2}{l}{LAMDA: a learning-assisted framework to accelerate FPGA design closure by autotuning FPGA toolflow configurations \cite{ustun2019lamda}. }  \\

                
     &   \multicolumn{2}{l}{CPU DSE: a reinforcement learning based automated DSE framework for DNN implementation on embedded CPUs \cite{de2020automated}.} \\
     
    
     \hline
     
     
    \end{tabular}
    \caption{A summary of enabling edge AI methodologies}
    \label{tab:methodology}
\end{table*}





==> tables/comparison_with_methods.tex <==
\renewcommand{\arraystretch}{1.1}
\begin{table*}[]
    \centering
    \caption{The comparison with other state-of-the-art quantization solutions.}
    \vspace{-8pt}
    \label{tab:imagenet_results}
    \setlength{\tabcolsep}{4.7mm}{
    \begin{tabular}{c|c|c|c|c|c|c}\Xhline{1.5pt}  \multirow{3}{*}{\textbf{Bitwidth}}&\multirow{3}{*}{\textbf{Methods}}&\multicolumn{5}{c}{\textbf{Datasets\&Models}}\\\cline{3-7}
    &&\multicolumn{1}{c|}{\textbf{MNIST}}&\multicolumn{1}{c|}{\textbf{Cifar10}~\cite{krizhevsky2009learning}}&\multicolumn{3}{c}{\textbf{ImageNet}~\cite{deng2009imagenet}}\\\cline{3-7}
    &&\multicolumn{1}{c|}{\textbf{LeNet5}}&\multicolumn{1}{c|}{\textbf{VGG-like}~\cite{simonyan2014vgg}}&\multicolumn{1}{c|}{\textbf{AlexNet}~\cite{alexnet}}&\multicolumn{1}{c|}{\textbf{ResNet18}~\cite{he2016resnet}}&\multicolumn{1}{c}{\textbf{MobileNetV2}~\cite{sandler2018mobilenetv2}}\\\Xhline{1.5pt}
    \textbf{32}&\textbf{FP32}&99.40&93.49&60.01/81.90&69.60/89.24&71.30/90.10\\\Xhline{1.0pt}
    \multirow{8}{*}{1}&{ReBNet\cite{ghasemzadeh2018rebnet}}&98.25&86.98&41.43/-&-&-\\
    &{BC~\cite{Binaryconnect}}&98.82&-&-&-&-\\
    &{BWN\cite{rastegari2016xnor}}&-&-&56.80/79.40&60.80/83.00&-\\
    &{BPWN\cite{TWNs}}&99.05&-&-&57.50/81.20&-\\
    &{ENN~\cite{ENN2017}}&-&-&57.00/79.70&64.80/86.20&-\\
    &{$\mu$L2Q~\cite{cheng2019uL2Q}}&99.06&89.02&-&66.24/86.00&-\\
    &\textbf{VecQ}&\textbf{99.34}&\textbf{90.39}&55.06/77.78&65.58/86.24&53.78/77.07\\\cline{2-7}
    &\textbf{Mean-Imp\footnotemark[3]}& 0.55& 2.39 & 3.32/-1.77&3.24/2.14&-/-
    \\\Xhline{1.0pt}
    \multirow{12}{*}{2}&{FP~\cite{gysel2016hardware}}&98.90&-&-&-&-\\
    &{TWN~\cite{TWNs}}&99.35&-&57.50/79.80\footnotemark[1]&61.80/84.20&-\\
    &{TC~\cite{Ternaryconnect}}&98.85&-&-&-&-\\
    &{TNN~\cite{alemdar2017ternary}}&98.33&-&-&-&-\\
    &{TTQ~\cite{zhu2016TTQ}}&-&-&57.50/79.70&66.60/87.20&-\\
    &{INQ~\cite{INQ2017}}&-&-&-&66.02/87.13&-\\
    &{ENN}&-&-&58.20/80.60&67.00/87.50&-\\
    &{TSQ~\cite{TSQ2018}}&-&-&58.00/80.50&-&-\\
    &{$\mu$L2Q}&99.12&89.50&-&65.60/86.12&-\\
    &{DC\footnotemark[4]}&-&-&-&-&58.07/81.24\\
    &\textbf{VecQ}&\textbf{99.53}&\textbf{92.94}&\textbf{59.31/81.01}&\textbf{68.23/88.10}&\textbf{64.67/85.24}\\\cline{2-7}
    &\textbf{Mean-Imp}& 0.62& 3.44 & 1.51/0.86&2.83/1.67&6.60/4.00
    \\\Xhline{1.0pt}
    \multirow{5}{*}{3}&{INQ}&-&-&-&68.08/88.36&-\\
    &{ENN}\footnotemark[2]&-&-&60.00/82.20&68.00/88.30&-\\
    &{DC}&-&-&-&-&68.00/87.96\\
    &\textbf{VecQ}&99.48&93.02&\textbf{60.36/82.40}&\textbf{68.79/88.45}&\textbf{69.13/88.35}\\\cline{2-7}
    &\textbf{Mean-Imp}& -& - & 0.36/0.20&0.75/0.12&1.13/0.39
    \\\Xhline{1.0pt}
    \multirow{6}{*}{4}&{FP}&99.10&-&-&-&-\\
    &{INQ}&-&-&-&68.89/89.01&-\\
    &{$\mu$L2Q}&99.12&89.80&-&65.92/86.72&-\\
    &{DC}&-&-&-&-&71.24/89.93\\
    &\textbf{VecQ}&\textbf{99.47}&\textbf{93.27}&61.21/82.94&\textbf{69.80}/\textbf{89.11}&\textbf{71.89/90.38}\\\cline{2-7}
    &\textbf{Mean-Imp}& 0.36& 3.47 & -/-&2.39/1.24&0.65/0.45
    \\\Xhline{1.0pt}
    \multirow{3}{*}{5}&{INQ}&-&-&57.39/80.46&68.98/89.10&-\\
    &\textbf{VecQ}&99.47&93.37&\textbf{61.65/83.19}&\textbf{69.98}/\textbf{89.15}&71.47/90.15\\\cline{2-7}
    &\textbf{Mean-Imp}& -& - & 3.26/2.73&1.00/0.05&-/-
    \\\Xhline{1.0pt}
    \multirow{3}{*}{6}
    &{HAQ}&-&-&-&-&66.75/87.32\\
    &\textbf{VecQ}&99.49&93.51&62.01/83.32&69.81/88.87&\textbf{72.23/90.61}\\\cline{2-7}
    &\textbf{Mean-Imp}& -& - & -/-&-/-&5.48/3.29
    \\\Xhline{1.0pt}
    \multirow{1}{*}{7}
    &\textbf{VecQ}&99.48&93.52&62.09/83.44&70.17/89.09&72.33/90.62
    \\\Xhline{1.0pt}
    \multirow{8}{*}{8}&{FP}&99.10&-&-&-&-\\
    &{$\mu$L2Q}&99.16&89.70&-&65.52/86.36&-\\
    &{QAT-c\footnotemark[5]}&-&-&-&-&71.10/-\\
    &{TQT-wt-th}&-&-&-&-&71.80/90.60\\
    &\textbf{VecQ}&\textbf{99.48}&\textbf{93.50}&62.22/83.54&\textbf{70.36/89.20}&\textbf{72.24/90.66}\\\cline{2-7}
    &\textbf{Mean-Imp}& 0.35& 3.80 & -/-&4.84/2.84&0.79/0.06
    \\\Xhline{1.5pt}
    \end{tabular}}\\\raggedright
    \footnotemark[1]{The results of TWN on AlexNet are from \cite{ENN2017}.}\\
    \footnotemark[2]{ENN adopts 2 bits shifting results noted as $\{-4,+4\}$~\cite{ENN2017}.}\\
    \footnotemark[3]{Mean-Imp denotes \textbf{Mean} of accuracy \textbf{Imp}rovement results compared to the state-of-the-art methods.}\\
    \footnotemark[4]{The results are from HAQ~\cite{wang2019haq}.}\\
    \footnotemark[5]{The results are from \cite{QAT_results}.}
    \vspace{-7pt}
\end{table*}

==> tables/comparison_with_methods_v2.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{table*}[]
    \flushleft
    \vspace{-20pt}
    \caption{The comparison with other state-of-the-art quantization solutions.}
    \label{tab:imagenet_results}
    \setlength{\tabcolsep}{7.7mm}{\begin{tabular}{lll}
    \Xhline{1.5pt}
    \textbf{Methods}& \textbf{Bits (W/A)} & \textbf{Accuray}\\\hline\hline
    \multicolumn{3}{c}{Lenet5 on MNIST}\\\Xhline{0.5pt}
         Float32& 32/32 & 99.40 \\\Xhline{0.5pt}
         BC \cite{Binaryconnect}& 1/32 & 98.71\\
         BPWN~\cite{TWNs} & 1/32 & 99.05\\
         $\mu$L2Q~\cite{cheng2019uL2Q}& 1/32 & 99.06\\
         \textbf{VecQ} & 1/32 & \textbf{99.34}\\\Xhline{0.5pt}
         Mean-Imp\footnotemark[4]& - & 0.40\\\Xhline{1pt}
         FP~\cite{gysel2016hardware} & 2/32 & 98.90\\
         TWN~\cite{TWNs} & 2/32 & 99.35\\
         $\mu$L2Q~\cite{cheng2019uL2Q}& 2/32 & 99.12\\
         \textbf{VecQ} & 2/32 & \textbf{99.53}\\\Xhline{0.5pt}
         Mean-Imp& - & 0.41\\\Xhline{1pt}
         FP & 4/32 & 99.10\\
         $\mu$L2Q& 4/32 & 99.12\\
         \textbf{VecQ} & 4/32 & \textbf{99.47}\\\Xhline{0.5pt}
         Mean-Imp& - & 0.36\\\Xhline{1pt}
         FP & 8/32 & 99.10\\
         $\mu$L2Q& 8/32 & 99.16\\
         \textbf{VecQ} & 8/32 & \textbf{99.48}\\\Xhline{0.5pt}
         Mean-Imp& - & 0.35\\
    \Xhline{1.5pt}
    \multicolumn{3}{c}{VGG-like~\cite{simonyan2014vgg} on Cifar10~\cite{krizhevsky2009learning}}\\\Xhline{0.5pt}
         Float32& 32/32 & 93.49 \\\Xhline{0.5pt}
         ReBNet~\cite{ghasemzadeh2018rebnet}& 1/3 & 86.98\\
         BC~\cite{Binaryconnect}& 1/32 & 88.44\\
         $\mu$L2Q& 1/32 & 89.02\\
         \textbf{VecQ} & 1/32 & \textbf{90.39}\\\Xhline{0.5pt}
         Mean-Imp& - & 2.24\\\Xhline{1pt}
         TC~\cite{Ternaryconnect} & 2/32 & 89.07\\
         TNN~\cite{alemdar2017ternary}& 2/2 & 87.89\\
         $\mu$L2Q& 2/32 & 89.50\\
         \textbf{VecQ} & 2/32 & \textbf{92.94}\\\Xhline{0.5pt}
         Mean-Imp& - & 4.12\\\Xhline{1pt}
         $\mu$L2Q& 4/32 & 89.80\\
         \textbf{VecQ} & 4/32 & \textbf{93.27}\\\Xhline{0.5pt}
         Mean-Imp& - & 3.47\\\Xhline{1pt}
         $\mu$L2Q& 8/32 & 89.70\\
         \textbf{VecQ} & 8/32 & \textbf{93.5}\\\Xhline{0.5pt}
         Mean-Imp& - & 3.80\\
    \Xhline{1.5pt}
    \multicolumn{3}{c}{AlexNet~\cite{alexnet} on ImageNet~\cite{deng2009imagenet}~(Top1/Top5)}\\\Xhline{0.5pt}
         Float32& 32/32 & 60.01/81.90 \\\Xhline{0.5pt}
         %1
         BWN~\cite{rastegari2016xnor}& 1/32 & 56.80/79.40\\
         ENN~\cite{ENN2017} & 1/32 & 57.00/79.70\\
         \textbf{VecQ} & 1/32 & 55.06/77.78\\\Xhline{0.5pt}
         Mean-Imp& - & -1.84/-1.91\\\Xhline{1pt}
         %2
         TWN\footnotemark[1] & 2/32 & 57.50/79.80\\
         TTQ~\cite{zhu2016TTQ} & 2/32 & 57.50/79.70 \\
         ENN & 2/32 & 58.20/80.60 \\
         TSQ~\cite{TSQ2018} & 2/2 & 58.00/80.50 \\
         \textbf{VecQ} & 2/32 & \textbf{59.31/81.01}\\\Xhline{0.5pt}
         Mean-Imp& - & 1.51/0.86\\\Xhline{1pt}
         %3
         ENN+2\footnotemark[2]&3/32&59.20/81.80\\
         ENN+4\footnotemark[3]&3/32&60.00/82.40\\
         \textbf{VecQ} & 3/32 & \textbf{60.36/82.40}\\\Xhline{0.5pt}
         Mean-Imp& - &0.76/0.30 \\
    \Xhline{1.5pt}
    \end{tabular}}~~~
    %ResNet18
    \begin{tabular}{lll}
    \Xhline{1.5pt}
    \textbf{Methods}& \textbf{Bits (W/A)} & \textbf{Accuray}\\\hline\hline
    \multicolumn{3}{c}{ResNet18~\cite{he2016resnet} on ImageNet~\cite{deng2009imagenet}~(Top1/Top5)}\\\Xhline{0.5pt}
    Float32& 32/32 & 69.60/89.24 \\\Xhline{0.5pt}
         %1
    BWN& 1/32 & 60.80/83.00\\
    BPWN & 1/32 & 57.50/81.20\\
    ENN & 1/32 & 64.80/86.20\\
    $\mu$L2Q&1/32&66.24/86.00\\
    \textbf{VecQ}&1/32 & 65.58/86.24\\\Xhline{0.5pt}
    Mean-Imp& - &3.25/2.14 \\\Xhline{1pt}
    %2
    TWN & 2/32 & 61.80/84.20\\
    TTQ & 2/32 & 66.60/87.20\\
    INQ~\cite{INQ2017} & 2/32 & 66.02/87.12\\
    ENN & 2/32 & 67.00/87.50\\
    $\mu$L2Q & 2/32 & 65.60/86.12\\
    \textbf{VecQ}&2/32 & \textbf{68.23/88.10}\\\Xhline{0.5pt}
    Mean-Imp& - &2.83/1.67 \\\Xhline{1pt}
    %3
    INQ & 3/32 & 68.02/87.12\\
    ENN+2 & 3/32 & 67.50/87.50\\
    ENN+4 & 3/32 & 68.00/88.30\\
    \textbf{VecQ}&3/32 & \textbf{68.79/88.45}\\\Xhline{0.5pt}
    Mean-Imp& - &0.93/0.26 \\\Xhline{1pt}
    %4
    INQ & 4/32 & 68.89/89.01\\
    $\mu$L2Q & 4/32 & 65.92/86.72\\
    \textbf{VecQ}&4/32 & \textbf{68.96}/88.52\\\Xhline{0.5pt}
    Mean-Imp& - &1.55/0.65 \\\Xhline{1pt}
    %5
    INQ & 5/32 & 68.98/89.10\\
    \textbf{VecQ}&5/32 & \textbf{69.15}/88.57\\\Xhline{0.5pt}
    Mean-Imp& - &0.17/-0.53 \\\Xhline{1pt}
    %8
    $\mu$L2Q & 8/32 & 65.52/86.36\\
    \textbf{VecQ}&8/32 & \textbf{70.36/89.20}\\\Xhline{0.5pt}
    Mean-Imp& - &4.84/2.84 \\
    % MobileNetV2
    \Xhline{1.5pt}
    \multicolumn{3}{c}{MobileNetV2~\cite{sandler2018mobilenetv2} on ImageNet~\cite{deng2009imagenet}~(Top1/Top5)}\\\Xhline{0.5pt}
    Float32& 32/32 & 71.30/90.10 \\\Xhline{0.5pt}
    %2
    DC\footnotemark[5]~\cite{han2015deep} & 2/32 & 58.07/81.24\\
    \textbf{VecQ} & 2/32 & \textbf{64.67/85.24}\\\Xhline{0.5pt}
    Mean-Imp& - &6.60/4.00 \\\Xhline{1pt}
    %3
    DC & 3/32 & 68.00/87.96\\
    \textbf{VecQ} & 3/32 & \textbf{69.13/88.35}\\\Xhline{0.5pt}
    Mean-Imp& - &1.13/0.39 \\\Xhline{1pt}
    %4
    DC & 4/32 & 71.24/89.93\\
    \textbf{VecQ} & 4/32 & \textbf{71.89/90.38}\\\Xhline{0.5pt}
    Mean-Imp& - &0.65/0.45 \\\Xhline{1pt}
    %6
    HAQ~\cite{wang2019haq} & 6/32 & 66.75/87.32\\
    \textbf{VecQ} & 6/32 & \textbf{72.23/90.61}\\\Xhline{0.5pt}
    Mean-Imp& - &5.48/3.29 \\\Xhline{1pt}
    %8
    QAT-t\footnotemark[6]~\cite{QAT} & 8/8 & 70.09/-\\
    QAT-c & 8/8 & 71.10/-\\
    TQT-wt~\cite{TQT} & 8/8 & 68.20/89.00\\
    TQT-wt-th & 8/8 & 71.80/90.60\\
    \textbf{VecQ} & 8/32 & \textbf{72.24/90.66}\\\Xhline{0.5pt}
    Mean-Imp& - &1.94/0.86 \\
    \Xhline{1.5pt}
    \end{tabular}\\\raggedright
    \footnotemark[1]{The results of TWN on AlexNet are from ENN \cite{ENN2017}.}
    \footnotemark[2]{ENN-3+2 means the 1bit shift results are noted as $\{-2,+2\}$ in ENN \cite{ENN2017}.}
    \footnotemark[3]{ENN-3+4 means the 2bits shift results are noted as $\{-4,+4\}$ in ENN \cite{ENN2017}.}
    \footnotemark[4]{Mean-Imp denotes \textbf{Mean} of accuracy \textbf{Imp}rovement results compared to the state-of-the-art methods.}
    \footnotemark[5]{The results are from HAQ~\cite{wang2019haq}.}
    \footnotemark[6]{The results are from \cite{QAT_results}.}
\end{table*}

==> tables/configures_of_comparing_works.tex <==
\begin{table}[]
\centering
\caption{\label{tab:comparison_methods_config}
Detailed settings of the quantization methods collected from the literature.}
\vspace{-5pt}
\resizebox{0.49\textwidth}{110pt}{
\setlength\tabcolsep{3pt} % default value: 6pt
\begin{tabular}{l|ccc|ccc|ccc}\Xhline{1.5pt}
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Methods}}} & \multicolumn{3}{c|}{\textbf{Weights}} & \multicolumn{3}{c|}{\textbf{Activation}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{FConv}}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{IFC}}} & \multicolumn{1}{c}{\multirow{2}{*}{\textbf{LFC}}} \\\cline{2-7}
\multicolumn{1}{c|}{} & \multicolumn{1}{c}{\textbf{Bits}} & \multicolumn{1}{c}{\textbf{SFB}} & \multicolumn{1}{c|}{\textbf{SFN}} & \multicolumn{1}{c}{\textbf{Bits}} & \multicolumn{1}{c}{\textbf{SFB}} & \multicolumn{1}{c|}{\textbf{SFN}} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{1}{c}{} \\\Xhline{1.5pt}
ReBNet~\cite{ghasemzadeh2018rebnet} & 1 & 32 & 1 & 3 & 32 & 3 & - & Y & N \\
BC~\cite{Binaryconnect} & 1 & - & 0 & 32 & - & - & - & - & - \\
BWN~\cite{rastegari2016xnor} & 1 & 32 & 1 & 32 & - & - & - & - & - \\
BPWN~\cite{TWNs} & 1 & 32 & 1 & 32 & - & - & - & N & N \\
TWN~\cite{TWNs} & 2 & 32 & 1 & 32 & - & - & - & N & N \\
TC~\cite{Ternaryconnect} & 2 & - & 0 & 32 & - & - & - & - & - \\
TNN~\cite{alemdar2017ternary} & 2 & - & 0 & 2 & - & 0 & - & - & - \\
TTQ~\cite{zhu2016TTQ} & 2 & 32 & 2 & 32 & - & - & N & Y & N \\
INQ~\cite{INQ2017} & 2,3,4,5 & - & 0 & 32 & - & - & - & - & - \\
FP~\cite{gysel2016hardware} & 2,4,8 & - & 0 & 32 & - & - & - & N & N \\
uL2Q~\cite{cheng2019uL2Q} & 1,2,4,8 & 32 & 1 & 32 & - & - & Y & Y & 8 \\
ENN~\cite{ENN2017} & 1,2,3 & 32 & 1 & 32 & - & - & - & - & - \\
TSQ~\cite{TSQ2018} & 2 & 32 & c\footnotemark[4] & 2 & 32 & 2 & N & Y & N \\
DC~\cite{han2015deep}\footnotemark[2] & 2,3,4 & 32 & 4,8,16 & 32 & - & - & 8 & - & 1 \\
HAQ~\cite{wang2019haq}\footnotemark[3] & flexible & 32 & 1 & 32 & - & - & 8 & - & 1 \\
QAT~\cite{QAT} & 8 & 32 & 1 & 8 & 32 & 1 & N & - & N \\
TQT~\cite{TQT} & 8 & - & 1 & 8 & - & 1 & 8 & - & 8 \\\Xhline{0.5pt}
\textbf{VecQ} & \textbf{1-8} & \textbf{32} & \textbf{1} & \textbf{32,8} & \textbf{-,32} & \textbf{-,1} & \textbf{Y} & \textbf{Y} & \textbf{Y}\\\Xhline{1.5pt}
\end{tabular}}\\\raggedright
\footnotemark[1]{
\textbf{Weights} and \textbf{Activation} denote the quantized data of the model. 
\textbf{Bits} refer to quantized bitwidth of methods; \textbf{SFB} is the bitwidth for the scaling-factor; \textbf{SFN} is the number of the scaling-factors. \textbf{FConv}, \textbf{IFC} and \textbf{LFC} represent whether the \textbf{F}irst \textbf{Conv}olution layer, the \textbf{I}nternal \textbf{F}ully-\textbf{C}onnected layers and the \textbf{L}ast \textbf{F}ully-\textbf{C}onnected layer are quantized.} \\
\footnotemark[2]{The results of DC are from~\cite{wang2019haq}.} \\
\footnotemark[3]{HAQ is a mix-precision method; results here are from the experiments that only quantize the weight data.} \\
\footnotemark[4]{TSQ introduces a floating-point scaling factor for each convolutional kernel, so the SFN equals to the number of kernels.}
\vspace{-10pt}
\end{table}

==> tables/sod.tex <==
\begin{table*}[t!]
\centering
\caption{The salient object detection results.}
\vspace{-6pt}
\label{tab:sod_results}
\resizebox{1.0\textwidth}{27mm}{
\setlength\tabcolsep{1pt} % default value: 6pt
\begin{tabular}{l|l||cccc|cccc|cccc|cccc|cccc|cccc}\Xhline{1.2pt}
                  & \textbf{Datasets} & \multicolumn{4}{c|}{\textbf{MSRA10K-test}}                            & \multicolumn{4}{c|}{\textbf{ECSSD}}                                   & \multicolumn{4}{c|}{\textbf{HKU-IS}}                                  & \multicolumn{4}{c|}{\textbf{DUTs}}                                    & \multicolumn{4}{c|}{\textbf{DUT-OMRON}}                               & \multicolumn{4}{c}{\textbf{THUR15K}}                                   \\\Xhline{1.2pt}
\textbf{Model}    & \textbf{Size (M)} & \textbf{MAE $\downarrow$}    & \textbf{MaxF $\uparrow$}   & \textbf{S $\uparrow$}      & \textbf{E $\uparrow$}      & \textbf{MAE $\downarrow$}    & \textbf{MaxF $\uparrow$}   & \textbf{S $\uparrow$}      & \textbf{E $\uparrow$}     & \textbf{MAE $\downarrow$}    & \textbf{MaxF $\uparrow$}   & \textbf{S $\uparrow$}      & \textbf{E $\uparrow$}     & \textbf{MAE $\downarrow$}    & \textbf{MaxF $\uparrow$}   & \textbf{S $\uparrow$}      & \textbf{E $\uparrow$}     & \textbf{MAE $\downarrow$}    & \textbf{MaxF $\uparrow$}           & \textbf{S $\uparrow$}              & \textbf{E  $\uparrow$}              & \textbf{MAE $\downarrow$}             &  \textbf{MaxF $\uparrow$}            & \textbf{S $\uparrow$}             & \textbf{E  $\uparrow$  }            \\\Xhline{1.2pt}
\textbf{Unet}                        & 139.37                      & 0.030                                 & 0.945                                  & 0.931                                  & 0.962                                  & 0.057                                 & 0.909                                  & 0.886                                  & 0.914          & 0.045                                 & 0.907                                  & 0.884                                  & 0.930          & 0.060                                 & 0.896                                  & 0.865                                  & 0.874          & 0.070                                 & 0.804          & 0.803                                  & 0.829                                  & 0.077                                  & 0.769         & 0.807                                  & 0.816                                  \\
\textbf{Unet*}                       & \emph{ 9.05} & 0.032                                 & 0.940                                  & 0.926                                  & 0.959                                  & 0.064                                 & 0.896                                  & 0.871                                  & 0.906          & 0.050                                 & 0.893                                  & 0.870                                  & 0.923          & 0.065                                 & 0.885                                  & 0.852                                  & 0.871          & 0.071                                 & 0.793          & 0.795                                  & 0.835                                  & 0.081                                  & 0.749         & 0.797                                  & 0.815                                  \\\Xhline{0.5pt}
\textbf{Bias}                        & 93.51\%                      & \textbf{-0.002}                       & \textbf{0.004}                         & \textbf{0.005}                         & \textbf{0.003}                         & \textbf{-0.007}                       & 0.013                                  & 0.015                                  & \textbf{0.008} & \textbf{-0.005}                       & 0.014                                  & 0.015                                  & \textbf{0.007} & \textbf{-0.005}                       & 0.011                                  & 0.012                                  & \textbf{0.003} & \textbf{-0.001}                       & 0.011          & \textbf{0.008}                         & \emph{\textbf{-0.006}} & \textbf{-0.005}                        & 0.020         & \textbf{0.010}                         & \textbf{0.001}                         \\\Xhline{1.2pt}
\textbf{FPN}                         & 109.38                      & 0.043                                 & 0.920                                  & 0.899                                  & 0.949                                  & 0.070                                 & 0.882                                  & 0.854                                  & 0.901          & 0.059                                 & 0.875                                  & 0.848                                  & 0.911          & 0.072                                 & 0.875                                  & 0.835                                  & 0.861          & 0.081                                 & 0.777          & 0.772                                  & 0.812                                  & 0.087                                  & 0.750         & 0.778                                  & 0.804                                  \\
\textbf{FPN*}                        & \emph{ 7.2}  & 0.038                                 & 0.935                                  & 0.920                                  & 0.955                                  & 0.070                                 & 0.889                                  & 0.866                                  & 0.897          & 0.059                                 & 0.879                                  & 0.859                                  & 0.908          & 0.070                                 & 0.878                                  & 0.850                                  & 0.859          & 0.080                                 & 0.772          & 0.786                                  & 0.809                                  & 0.089                                  & 0.739         & 0.789                                  & 0.796                                  \\\Xhline{0.5pt}
\textbf{Bias} & 93.42\%                      & \emph{\textbf{0.005}} & \emph{\textbf{-0.015}} & \emph{\textbf{-0.022}} & \emph{\textbf{-0.006}} & \emph{\textbf{0.000}} & \emph{\textbf{-0.007}} & \emph{\textbf{-0.012}} & \textbf{0.004} & \emph{\textbf{0.001}} & \emph{\textbf{-0.005}} & \emph{\textbf{-0.011}} & \textbf{0.004} & \emph{\textbf{0.002}} & \emph{\textbf{-0.003}} & \emph{\textbf{-0.015}} & \textbf{0.003} & \emph{\textbf{0.001}} & \textbf{0.004} & \emph{\textbf{-0.014}} & \textbf{0.003}                         & \emph{\textbf{-0.002}} & 0.011         & \emph{\textbf{-0.011}} & \textbf{0.007}    
 \\\Xhline{1.2pt}
\textbf{Linknet}                     & 109.8                       & 0.032                                 & 0.942                                  & 0.928                                  & 0.959                                  & 0.060                                 & 0.905                                  & 0.882                                  & 0.911          & 0.048                                 & 0.900                                  & 0.878                                  & 0.927          & 0.062                                 & 0.892                                  & 0.861                                  & 0.871          & 0.071                                 & 0.801          & 0.799                                  & 0.825                                  & 0.079                                  & 0.760         & 0.803                                  & 0.814                                  \\
\textbf{Linknet*}                    & \emph{ 7.24} & 0.034                                 & 0.939                                  & 0.923                                  & 0.959                                  & 0.068                                 & 0.891                                  & 0.865                                  & 0.902          & 0.054                                 & 0.887                                  & 0.860                                  & 0.920          & 0.068                                 & 0.883                                  & 0.847                                  & 0.870          & 0.072                                 & 0.788          & 0.787                                  & 0.833                                  & 0.082                                  & 0.746         & 0.794                                  & 0.818                                  \\\Xhline{0.5pt}
\textbf{Bias}                        & 93.40\%                      & \textbf{-0.002}                       & \textbf{0.003}                         & \textbf{0.004}                         & \textbf{0.001}                         & \textbf{-0.008}                       & 0.014                                  & 0.017                                  & \textbf{0.008} & \textbf{-0.005}                       & 0.013                                  & 0.018                                  & \textbf{0.006} & \textbf{-0.005}                       & 0.010                                  & 0.014                                  & \textbf{0.001} & \textbf{-0.001}                       & 0.014          & 0.012                                  & \emph{\textbf{-0.008}} & \textbf{-0.002}                        & 0.014         & \textbf{0.009}                         & \emph{\textbf{-0.004}} \\\Xhline{1.2pt}
\textbf{UNet++}                      & 143.81                      & 0.029                                 & 0.948                                  & 0.933                                  & 0.964                                  & 0.056                                 & 0.910                                  & 0.888                                  & 0.915          & 0.044                                 & 0.909                                  & 0.887                                  & 0.930          & 0.059                                 & 0.897                                  & 0.867                                  & 0.876          & 0.070                                 & 0.805          & 0.805                                  & 0.829                                  & 0.076                                  & 0.769         & 0.810                                  & 0.818                                  \\
\textbf{UNet++*}                     & \emph{ 9.35} & 0.033                                 & 0.939                                  & 0.926                                  & 0.958                                  & 0.065                                 & 0.895                                  & 0.872                                  & 0.905          & 0.052                                 & 0.890                                  & 0.868                                  & 0.919          & 0.066                                 & 0.884                                  & 0.854                                  & 0.867          & 0.075                                 & 0.785          & 0.792                                  & 0.822                                  & 0.082                                  & 0.750         & 0.797                                  & 0.811                                  \\\Xhline{0.5pt}
\textbf{Bias}                        & 93.50\%                      & \textbf{-0.004}                       & \textbf{0.008}                         & \textbf{0.007}                         & \textbf{0.007}                         & \textbf{-0.009}                       & 0.015                                  & 0.016                                  & 0.010          & \textbf{-0.008}                       & 0.019                                  & 0.018                                  & 0.011          & \textbf{-0.007}                       & 0.013                                  & 0.013                                  & \textbf{0.009} & \textbf{-0.005}                       & 0.020          & 0.013                                  & \textbf{0.007}                         & \textbf{-0.006}                        & 0.019         & 0.013                                  & \textbf{0.007}                         \\\Xhline{1.2pt}
\end{tabular}}\\\flushleft
\vspace{-5pt}
\footnotemark[1]{S and E stand for S-measure and E-measure, respectively. The $\uparrow$ indicates that the higher value shows better results and the $\downarrow$ is vise versa. The $*$ indicates the quantized models with VecQ-2 and the quantized model sizes are marked in \emph{italics}. \textbf{Bias} row lists the difference between the full-precision model and the quantized model. A negative value is better in S$\uparrow$, E$\uparrow$, and MaxF$\uparrow$ column but worse in the MAE$\downarrow$ column}.
\vspace{-6pt}
\end{table*}


==> tables/vecq-quantization-results-table-v2.tex <==
\begin{table*}[t!]
    \centering
    \caption{The accuracy and model size with different bitwidth targets.}
    \vspace{-8pt}
    \label{tab:vecq_under_bit_width}
    \setlength{\tabcolsep}{3mm}{\begin{tabular}{c|cc|cc|cc|cc|cc}
    \Xhline{1.5pt}
    \multirow{2}{*}{W/A\footnotemark[1]}& \multicolumn{2}{c|}{LeNet5 } & \multicolumn{2}{c|}{VGG-like~\cite{simonyan2014vgg}} & \multicolumn{2}{c|}{Alexnet~\cite{alexnet}} & \multicolumn{2}{c|}{ResNet-18~\cite{he2016resnet}} & \multicolumn{2}{c}{MobileNetV2~\cite{sandler2018mobilenetv2}} \\\cline{2-11}
    &Size(M)&Acc&Size(M)&Acc&Size(M)&Top1/Top5&Size(M)&Top1/Top5&Size(M)&Top1/Top5\\\Xhline{1.5pt}
    32/32&6.35&99.40&20.44&93.49&194.10&60.01/81.90\footnotemark[2]&44.63&69.60/89.24\footnotemark[3]
    &13.50&71.30/90.10\footnotemark[4]\\\Xhline{0.5pt}
    1/32&0.21&99.34&0.67&90.39& 6.21&55.06/77.78& 1.45&65.58/86.24&0.67&53.78/77.07\\
    2/32&\textbf{0.41}&\textbf{99.53}&1.31&92.94&12.27&59.31/81.01& 2.68&68.23/88.10&1.09&64.67/85.24\\
    3/32&0.60&99.48&1.94&93.02&18.33&60.36/82.40& 4.24&68.79/88.45&1.50&69.13/88.35\\
    4/32&0.80&99.47&2.58&93.27&24.39&61.21/82.94& 5.63&69.80/89.11&1.92&71.89/90.38\\
    5/32&1.00&99.47&3.22&93.37&30.45&61.65/83.19& 7.02&69.98/89.15&2.33&71.47/90.15\\
    6/32&1.20&99.49&3.86&93.51&36.51&62.01/83.32& 8.42&69.81/88.97&2.74&72.23/90.61\\
    7/32&1.40&99.48&\textbf{4.49}&\textbf{93.52}&42.57&62.09/83.44& 9.81&70.17/89.09&\textbf{3.16}&\textbf{72.33/90.62}\\
    8/32&1.60&99.48&5.13&93.50&\textbf{48.63}&\textbf{62.22/83.54}&\textbf{11.20}&\textbf{70.36/89.20}&3.57&72.24/90.66\\\Xhline{0.5pt}
    2/8 & 0.41 & 99.43 & 1.31 &  92.46 & 12.27 &58.04/80.21& 2.68 &67.91/88.30& 1.09 &63.34/84.42\\
    4/8 & 0.80 & 99.53 & 2.58 & 93.37 & 24.39  &61.22/83.24& 5.63 &68.41/88.76&1.92 &71.40/90.41\\
    8/8 & 1.60 & 99.44 & 5.13 & 93.55 &48.63&61.60/83.66& 11.20 &69.86/88.90& 3.57 &72.11/90.68\\
    \Xhline{1.5pt}
    \end{tabular}}\\\raggedright
    \footnotemark[1]{W/A denotes the quantizing bits of weights and activation respectively.}\\
    \footnotemark[2]{Results of AlexNet with Batch Normalization layers are cited from \cite{simon2016cnnmodels}.}\\
    \footnotemark[3]{Results of ResNet18 are cited from \cite{gross2016training}.}\\
    \footnotemark[4]{Results are cited from the document of Keras \cite{chollet2015keras}.}
    \vspace{-10pt}
\end{table*}

==> tables/vecq-quantization-results-table.tex <==
\begin{table*}[t!]
    \centering
    \caption{The accuracy and model size with different bitwidth targets.}
    \label{tab:vecq_under_bit_width}
    \setlength{\tabcolsep}{2.5mm}{\begin{tabular}{c|cc|cc|ccc|ccc|ccc}
    \Xhline{1.5pt}
    \multirow{2}{*}{Bits}& \multicolumn{2}{c|}{LeNet5} & \multicolumn{2}{c|}{VGG-like~\cite{simonyan2014vgg}} & \multicolumn{3}{c|}{Alexnet~\cite{alexnet}} & \multicolumn{3}{c|}{ResNet-18~\cite{he2016resnet}} & \multicolumn{3}{c}{MobileNetV2~\cite{sandler2018mobilenetv2}} \\\cline{2-14}
    &Size(M)&Acc&Size(M)&Acc&Size(M)&Top1&Top5&Size(M)&Top1&Top5&Size(M)&Top1&Top5\\\Xhline{1.5pt}
    32&6.35&99.4&20.44&93.49&194.10&60.01\footnotemark[1]&81.90\footnotemark[1]&44.63&69.60\footnotemark[2]&89.24\footnotemark[2]
    &13.50&71.30\footnotemark[3]&90.10\footnotemark[3]\\\Xhline{0.5pt}
    1&0.21&99.34&0.67&90.39& 6.21&55.06&77.78& 1.45&65.58&86.24&0.67&53.78&77.07\\
    2&0.41&99.53&1.31&92.94&12.27&59.31&81.01& 2.68&68.23&88.10&1.09&64.67&85.24\\
    3&0.60&99.48&1.94&93.02&18.33&60.36&82.40& 4.24&68.79&88.45&1.50&69.13&88.35\\
    4&0.80&99.47&2.58&93.27&24.39&61.21&82.94& 5.63&68.96&88.52&1.92&71.89&90.38\\
    5&1.00&99.47&3.22&93.37&30.45&61.65&83.19& 7.02&69.41&88.77&2.33&71.47&90.15\\
    6&1.20&99.49&3.86&93.51&36.51&62.01&83.32& 8.42&69.81&88.97&2.74&72.23&90.61\\
    7&1.40&99.48&4.49&93.52&42.57&62.09&83.44& 9.81&70.17&89.09&3.16&72.33&90.62\\
    8&1.60&99.48&5.13&93.50&48.63&62.22&83.54&11.20&70.36&89.20&3.57&72.24&90.66\\
    \Xhline{1.5pt}
    \end{tabular}}\\\raggedright
    \footnotemark[1]{Results of AlexNet with Batch Normalization layers are cited from \cite{simon2016cnnmodels}.}\\
    \footnotemark[2]{Rsults of ResNet18 are cited from \cite{gross2016training}.}\\
    \footnotemark[3]{Results are cited from the document of keras \cite{chollet2015keras}.}
\end{table*}
